A Framework to Estimate Life Cycle Emissions for Vehicle-Integrated Photovoltaic Systems

This paper presents a framework to estimate the environmental impact of solar electric vehicles, accounting for the emissions caused by photovoltaic system production as well as vehicle use. We leverage a cradle-to-gate life cycle assessment to estimate the greenhouse gas emissions of the vehicle-integrated photovoltaic system, from the raw material extraction to the final panel assembly, including the effect of the electricity mix both at the factory location and in the country of use. %the vehicle's life cycle, considering both Furthermore, we modify an existing optimization framework for battery electric vehicles to optimally design a solar electric vehicle and estimate its energy consumption. We showcase our framework by analyzing a case study where the mono-crystalline silicon extraction and refinement processes occur in China, while the final assembly of the panel is in The Netherlands, generating 118 kg of CO2 equivalents per square meter of solar panel. The results suggest that it is generally beneficial to operate solar electric vehicles in countries with a high irradiation index. However, when the local electricity mix already displays a low carbon intensity, the additional emissions introduced by the panel are unnecessary, requiring a longer vehicle lifetime to reach an advantageous emission balance.

==> Report/Titlepage.tex <==
\begin{titlepage}
	\centering
	\vspace*{0.5 cm}
	\includegraphics[width = 120mm]{Figures/Logo.eps}\\[0.5 cm]		% University Logo
	\textsc{\LARGE Eindhoven University of Technology}\\[2.0 cm]% University Name
	\textsc{\Large Master thesis}\\[0.5 cm]							% Course Code
%	\textsc{\large Graduation project}\\[0.5 cm]			% Course Name
	% 	{\bfseries Department of Mechanical Engineering\\}
	\rule{\linewidth}{0.2 mm} \\[0.4 cm]
	{\huge\bfseries Maximum-distance Race Strategies for a Fully Electric Endurance Race Car\\}
	%{\huge\bfseries \hl{Report Title Continuation} \\ }
	\rule{\linewidth}{0.2 mm} \\[1.5 cm]
	
	
	\begin{minipage}{0.4\textwidth}
		% \vspace{0.5cm}
		%\includegraphics[width=0.7\linewidth]{Figures/cover.png}\\[10pt]
		\centering
		% {\Large\bfseries Authors }\\[5pt]
		%\begin{table}[H]
		% \centering
		%   \label{authors}
		
		%  \begin{minipage}{0.4\textwidth}
			\begin{flushright} \normalsize
				
				Master \\
				Department \\
				Research group \\[1cm]
				\emph{Authors}\\
				\textsc{van Kampen} J.H.E.\\[1cm] % Name
			\end{flushright}
		\end{minipage}
		\hspace{1cm}
		\begin{minipage}{0.4\textwidth}
			\begin{flushleft} \normalsize
				
				Automotive Technology \\
				Mechanical Engineering \\
				Control Systems Technology\\[1cm]
				\emph{Student numbers} \\
				0952110\\ %student 
			\end{flushleft}
		\end{minipage}\\[2cm]
		\emph{Supervisor}\\
		dr. ir. M.R.U. Salazar Villalon\\[2cm]
		
		Eindhoven, \today
		
		%\begin{flushright}
		%    \vfill
		%	\hl{Supervised by}\\
		%	\hl{Name, \textsc{TU Eindhoven}}
		%\end{flushright}	
		\newpage
		\includegraphics[width=\linewidth]{Report/Code_of_conduct.pdf}
		\newpage
	\end{titlepage}

==> gensymb/README <==
============================================================

   gensymb – Generic symbols for both text and math mode

============================================================
Walter Schmidt

Keiran  Harcombe
kjh@harcombe.net
  
This LaTeX package provides generic commands
\degree, \celsius, \perthousand, \micro and \ohm, which
work both in text and math mode.  The package should
co-operate flawlessly with the well-known units.sty.
Various means are provided to fake the symbols or take
them from external symbol fonts, if they are not available
in the default fonts used in the document.  The package
makes optionally use of upgreek.sty.

The style files can be unpacked by running the particular
installation script (.ins) through LaTeX.  The files will 
be created immediately in the appropriate TDS directory
tex/latex/was, if this directory exists and the DOCSTRIP
tool is properly configured -- otherwise they are written
into the current directory.

The documentation of a package can be generated by running
the particular .dtx file through LaTeX.

==finis

